Compatibility-aware Heterogeneous Visual Search

We tackle the problem of visual search under resource constraints. Existing systems use the same embedding model to compute representations (embeddings) for the query and gallery images. Such systems inherently face a hard accuracy-efficiency trade-off: the embedding model needs to be large enough to ensure high accuracy, yet small enough to enable query-embedding computation on resource-constrained platforms. This trade-off could be mitigated if gallery embeddings are generated from a large model and query embeddings are extracted using a compact model. The key to building such a system is to ensure representation compatibility between the query and gallery models. In this paper, we address two forms of compatibility: One enforced by modifying the parameters of each model that computes the embeddings. The other by modifying the architectures that compute the embeddings, leading to compatibility-aware neural architecture search (CMP-NAS). We test CMP-NAS on challenging retrieval tasks for fashion images (DeepFashion2), and face images (IJB-C). Compared to ordinary (homogeneous) visual search using the largest embedding model (paragon), CMP-NAS achieves 80-fold and 23-fold cost reduction while maintaining accuracy within 0.3% and 1.6% of the paragon on DeepFashion2 and IJB-C respectively.

==> Tables/compatibility_bct.tex <==
\begin{table}[h!]
% \begin{adjustbox}{width=\columnwidth,center}
\centering
\small
\begin{tabular}{ccccc}
\toprule
Training & Scenario & Gallery & Query  & Acc. \\ \midrule

\multirow{3}{*}{Vanilla} & Symmetric & $w_{\phi,g}$ & $w_{\phi,g}$ & 86.7 \\ 
& Symmetric & $w_{\phi,q}$ & $w_{\phi,q}$ & 67.2 \\ 
& Asymmetric& $w_{\phi,g}$ & $w_{\phi,q}$ & 0 \\  \hdashline 
\multirow{3}{*}{BCT} & Symmetric& $w_{\phi,q,bct}$  & $w_{\phi,q,bct}$ & 75.5 \\ 
& Asymmetric& $w_{\phi,g}$ & $w_{\phi,q,bct}$ & 80.3 \\ 

% \multicolumn{1}{c|}{Model} & \multicolumn{2}{c|}{Without BCT} & \multicolumn{2}{c}{With BCT} \\
%  &   ($\phi_Q,\phi_Q$)  & ($\phi_Q,\phi_G$)   & ($\phi_Q,\phi_Q$) & ($\phi_Q,\phi_G$) \\ \midrule
% \begin{tabular}[c]{@{}l@{}}Resnet-101\\ (Gallery Net)\end{tabular} & 85.4 & - & - & - \\ \hline
% % ShuffleNet V1 (1x,g=1) & 58.8 & 0.0 & 67.2 & 74.5 \\
% % ShuffleNet V2& 61.0 & 0.0 & 66.8 & 74.8 \\ 
% MobileNet V1 & 50.0 & 0.0 & 67.0 & 73.0 \\
% MobileNet V2 & 66.7 & 0.0 & 75.4 & 80.3 \\
% MobileNet V3 & 67.2 & 0.0 & 74.3 & 79.9 \\ \hline
% ProxyLess (mobile) & 38.8 & 0.0 & 75.5 & 80.3 \\ \hline


\end{tabular}
% \end{adjustbox}
\caption{Achieving representational compatibility on 1:N face retrieval. We use a ResNet-101 and MobileNet V3 as the gallery and query models. Observe that training the query model with Vanilla training (Eq.) leads to $0\%$ accuracy while using BCT training (Eq.) leads to $80.3\%$ asymmetric accuracy. Also the latter model satisfies the AVS compatibility criterion. }
\label{tab:compat_bct}
\end{table}



==> Tables/computation_constrain.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\Huge
\centering
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{@{}lll|cc@{}}
\toprule
Gallery  & Query & Query & Fashion retreival & Face retreival \\
model & model & MFlops & top-10 search & 1:N search \\ \midrule
 % & &  & TAR(\%)@FAR=$10^{-4}$ & TNIR(\%)@FPRI=$10^{-2}$ \\
                            %   &                & ($\phi_Q,\phi_Q$)          & ($\phi_Q,\phi_G$)          & ($\phi_Q,\phi_Q$)         & ($\phi_Q,\phi_G$)        \\ \midrule
                               
ResNet-101 &     ResNet-101        & 7597            & 65.1               & 86.7  \\ \hline
\multirow{4}{*}{ResNet-101} 
% & ShuffleNetV2(x)             & 595             & 62.2                        & 74.4                \\
& MobileNetV1(1x)             & 579             & 62.3                        & 73.0                \\
& MobileNetV2(1x)             & 329                  & 60.4                     & 77.0                \\
& ProxyLess(mobile)             & 332                   & 62.1                      & 81.8                \\
% \small{CMP-NAS(C2S)}             & 321            & 81.6                  & 84.5                  & 83.3                 & 85.3                \\
& CMP-NAS-a   (ours)      & \textbf{327}                & \textbf{65.7}              & \textbf{85.1}                \\ \bottomrule
\multirow{2}{*}{ResNet-101} 
& MobileNetV3                   & 226         & 63                  & 80.4                   \\ 
& CMP-NAS-b   (ours)          &      \textbf{216}               & \textbf{64.9}     &         \textbf{84.1}            \\  \hline
\multirow{5}{*}{ResNet-101} 
& MobileNetV1(0.5x)  & 155  & 60.3  & 62.7 \\
& ShuffleNetV2(1x)   & 149  & 63.3  & 75.8 \\
& ShuffleNetV1(1x,g=1) & 148 & 62.6  & 76.0 \\
& MobileNetV2(0.5x)    & 100 & 62.0 & 73.1 \\
& CMP-NAS-c (ours)     & \textbf{94} & \textbf{64.8}  & \textbf{78.8} \\ \hline

% \small{ShuffleNet V2 (2x)}             & 595            & 66.6                  & 74.3                  & 68.2                 & 74.4                \\

\end{tabular}
\end{adjustbox}
\caption{Evaluating architectures search with \cmpnas for fashion retreival and face search tasks. We search models for three different flops targets: 100, 230 and 330 Mflops. The searched models outperform other architectures by $3-5\%$ on both the tasks.}
\label{tab:compat_nas_best}
\end{table}

==> Tables/parameter_compatibility.tex <==
\begin{table}[]
\begin{adjustbox}{width=\columnwidth,center}
\Large
\begin{tabular}{lc|cccc}
\toprule
Gallery & Query & Train & Finetune & BCT & KD \\ 
model & model & Scratch &  &  &  \\\midrule
% ResNet-101 & ResNet-101  & 87.3 & - & - & - \\ \hline
\multirow{2}{*} {\begin{tabular}[l]{@{}l@{}}Magnitude prune \\ ResNet-101 \end{tabular}}
& Magnitude prune & 83.4 & 83.9 & 85.6 & 85.8 \\
& Magnitude prune & 0 & 85.9 & 86.7 & 0 \\\hline
\multirow{2}{*} {\begin{tabular}[l]{@{}l@{}}Channel prune \\ ResNet-101 \end{tabular}}
& Channel prune & 83.2 & 84.4 & 85.6 & 86.4  \\
& Channel prune & 0 & 86.2 & 86.9 & 0  \\ \hline
\end{tabular}
\end{adjustbox}
\caption{Comparing techniques for achieving representatinal compatibility on 1:1 face verfication. The query model $\phi_Q$ is obtain by pruning $90\%$ of filters in each layer using two pruning methods. We see that for both methods, training the query model with BCT loss leads to the highest accuracy in the asymmetric setting.}
\label{tab:compatibility_comparison}
\end{table}

==> Tables/rewards.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\centering
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{@{}llc@{}}
\toprule
Reward & Formulation & Comment 
$\mathcal{R}_1$ & & 
$\mathcal{R}_2$ & & 
$\mathcal{R}_3$ & & 
% \textbf{\#} & Reward & \multicolumn{2}{c}{Encourages}    \\ 
%           &                             & \begin{tabular}[c]{@{}c@{}} $(\phi_Q,\phi_Q)$ \end{tabular} & \begin{tabular}[c]{@{}c@{}} $(\phi_G,\phi_G)$\end{tabular} \\ \midrule
% R1        & $M(\phi_Q,\phi_Q)$                         & \textcolor{ForestGreen}{$\uparrow$}          & Ignore          \\
% R2        & $M(\phi_Q,\phi_G)$                          & Ignore                                                                    & \textcolor{ForestGreen}{$\uparrow$}                                                                      \\ 
% R3        & $M(\phi_Q,\phi_Q) \times M(\phi_Q,\phi_G)$                     & \textcolor{ForestGreen}{$\uparrow$}                                                                      & \textcolor{ForestGreen}{$\uparrow$}                                                                       \\
% R4        & $M(\phi_Q,\phi_Q)+ M(\phi_Q,\phi_G)$                    & \textcolor{ForestGreen}{$\uparrow$}                                                                      & \textcolor{ForestGreen}{$\uparrow$}                                                                       \\  \bottomrule
\end{tabular}
\end{adjustbox}
\caption{Different rewards considered for Compat-NAS}
\label{tab:reward}
\end{table}
